Teacher Perception of Automatically Extracted Grammar Concepts for L2 Language Learning

One of the challenges of language teaching is how to organize the rules regarding syntax, semantics, or phonology of the language in a meaningful manner. This not only requires pedagogical skills, but also requires a deep understanding of that language. While comprehensive materials to develop such curricula are available in English and some broadly spoken languages, for many other languages, teachers need to manually create them in response to their students' needs. This process is challenging because i) it requires that such experts be accessible and have the necessary resources, and ii) even if there are such experts, describing all the intricacies of a language is time-consuming and prone to omission. In this article, we present an automatic framework that aims to facilitate this process by automatically discovering and visualizing descriptions of different aspects of grammar. Specifically, we extract descriptions from a natural text corpus that answer questions about morphosyntax (learning of word order, agreement, case marking, or word formation) and semantics (learning of vocabulary) and show illustrative examples. We apply this method for teaching the Indian languages, Kannada and Marathi, which, unlike English, do not have well-developed pedagogical resources and, therefore, are likely to benefit from this exercise. To assess the perceived utility of the extracted material, we enlist the help of language educators from schools in North America who teach these languages to perform a manual evaluation. Overall, teachers find the materials to be interesting as a reference material for their own lesson preparation or even for learner evaluation.

==> images/quality-study-questions.tex <==
\begin{table*}[t]
\small
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l|l}
    %\toprule
    Question & Answer Choices \\
    \midrule 
    1. Are the rules along with the accompanying examples  &
    a. precisely defining a linguistic distinction \\
    demonstrating the language property correctly?& b. too specific \\
    & c. too general \\
    & d. not corresponding to a real distinction in the language \\
    & e. cannot decide as incorrectly parsed \\
    
    \midrule
   2. What language learning level covers or should cover it?  & e.g. Textbook-1 \\
              
    \midrule
   3.1 If this material has already been covered,  & Yes/No \\
        could you still use some of our material & \\
        to enrich your existing material? & \\
    \midrule
    3.2 If the material is not already covered,  & Yes/No \\
    would you add this in your teaching & \\

    \end{tabular}
    }
    \caption{Questions asked to the Kannada experts for evaluating the quality and overall fit of the material.}
    \label{tab:qualityquestions}
    \vspace{-1em}
     %\vspace{-.3cm}
\end{table*}

==> images/relatedwordsummary.tex <==
\begin{table*}[t]
\small
    %\vspace{-.1cm}
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{c|l|c|c}
    \toprule
  Linguistic Phenomena &  Work & Rule-Type & Corpus Type   \\
    \midrule
  WordOrder & Ours & C+FG & Raw text\\
            & Grammar Matrix \cite{bender-etal-2002-grammar} & C+FG & IGT text* \\
            & \citet{lewis-xia-2008-automatically} & C &  IGT text \\
            & \citet{bender-etal-2013-towards} & C & IGT text \\
            & \citet{ostling-2015-word} & C & Raw text   \\
            & \citet{wang-eisner-2017-fine} & C & Raw text  \\
            & WALS \citet{wals} & C & Reference grammar* \\
  \midrule
  Case Marking & Ours & C+FG & Raw text \\
               & Grammar Matrix \cite{bender-etal-2002-grammar} & C+FG & IGT text* \\
               & WALS \citet{wals} & C & Reference grammar* \\
               & \citet{howell-etal-2017-inferring} & C & IGT text \\
    \midrule
    Agreement &  Ours & C+FG & Raw text \\
              & Grammar Matrix \cite{bender-etal-2002-grammar} & C+FG & IGT text* \\
              & \citet{chaudhary-etal-2020-automatic} & C+FG & Raw text \\
              
    \midrule 
    Sentence construction & \citet{hellan-2010-descriptive} & FG & IGT text* \\
   
    \end{tabular}
    }
    \caption{An overview of linguistic questions \emph{automatically} answered by our current work and existing related work. Some of them combine semi-automatic approaches with manually annotated resources, there are marked with *. Rule-Type  denotes the type of rule extracted for a language, C refers to coarse-grained  such as rules for canonical word order, FG refers to fine-grained i.e. rules extracted at a local level. 
    % \gn{I feel like it might be nicer if we had one column for each linguistic phenomenon like ``word order'', ``case marking'', ``morphological agreement'', ``morphological paradigms'' etc. And you could add a differernt symbol for ``canonical'' (``C''?) and fine-grained (``FG''?) in each column for each work that handles those things?} 
    }
    \label{tab:relatedwork}
    \vspace{-1em}
     %\vspace{-.3cm}
\end{table*}

==> images/systemoverview.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{images/Pipeline.pdf}
    \caption{An overview of the \textsc{AutoLEX} framework  (with Adj-N order in Spanish as an example). The example sentence translates to \emph{Four books were bought by the small girl}. First, we formulate a linguistic question (e.g.~regarding Adj-N order) as a binary classification task (e.g.~``whether the Adj comes before/after the N'). Next, we perform syntactic analysis on the raw text, from which we extract syntactic, lexical, and semantic features to construct the training data. Finally, we learn an interpretable model from which we  extract concise rules. 
    %\an{Might help if we number the steps of the process on the figure and also refer to these in the caption (and potentially in the main body text)?}
    %\aditi{added}
    }
    \label{fig:systemoverview}
    \vspace{-1em}
\end{figure*}

==> images/vocab-eval-example.tex <==
% district (NOUN)	"ಜಿಲ್ಲಾಡಳಿತ (jilladlit)
% ಜಿಲ್ಲಾ (jilla)
% ಜಿಲ್ಲಾಸ್ಪತ್ರೆ (jillaspatre)
% ಜಿಲ್ಲಾಧಿಕಾರಿ (jilladhikari)
% ತಾಲ್ಲೂಕು (talluku)"	20	"1 is district administration
% 2 is accurate
% 3 is district hospital
% 4 is district official
% 5 is taluk"

\begin{table*}[t]
\small
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{c|c|c}
    %\toprule
    English Word & Kannada Words & Expert Comment \\
    \midrule 
    temple (NOUN) & devsthan & district administration \\
                    & devalayas & district \\
                    & degul &  district hospital \\
                    & mandir & district official \\
                    
                    
    \midrule
   


    \end{tabular}
    }
    \caption{Vocabulary evaluation by Kannada experts. The Kannada word is written in the roman script for easy readability.\aditi{ask Arun/Ashwin for corrrect romanization of these words} }
    \label{tab:lingquestions}
    \vspace{-1em}
     %\vspace{-.3cm}
\end{table*}
